Generalizable Pedestrian Detection: The Elephant In The Room

Pedestrian detection is used in many vision based applications ranging from video surveillance to autonomous driving. Despite achieving high performance, it is still largely unknown how well existing detectors generalize to unseen data. This is important because a practical detector should be ready to use in various scenarios in applications. To this end, we conduct a comprehensive study in this paper, using a general principle of direct cross-dataset evaluation. Through this study, we find that existing state-of-the-art pedestrian detectors, though perform quite well when trained and tested on the same dataset, generalize poorly in cross dataset evaluation. We demonstrate that there are two reasons for this trend. Firstly, their designs (e.g. anchor settings) may be biased towards popular benchmarks in the traditional single-dataset training and test pipeline, but as a result largely limit their generalization capability. Secondly, the training source is generally not dense in pedestrians and diverse in scenarios. Under direct cross-dataset evaluation, surprisingly, we find that a general purpose object detector, without pedestrian-tailored adaptation in design, generalizes much better compared to existing state-of-the-art pedestrian detectors. Furthermore, we illustrate that diverse and dense datasets, collected by crawling the web, serve to be an efficient source of pre-training for pedestrian detection. Accordingly, we propose a progressive training pipeline and find that it works well for autonomous-driving oriented pedestrian detection. Consequently, the study conducted in this paper suggests that more emphasis should be put on cross-dataset evaluation for the future design of generalizable pedestrian detectors. Code and models can be accessed at https://github.com/hasanirtiza/Pedestron.

==> sections/abstract.tex <==
\begin{abstract}
Pedestrian detection is used in many vision based applications ranging from video surveillance to autonomous driving. 
Despite achieving high performance, it is still largely unknown how well existing detectors generalize to unseen data.
To this end, we conduct a comprehensive study in this paper, using a general principle of direct cross-dataset evaluation.
Through this study, we find that existing state-of-the-art pedestrian detectors generalize poorly from one dataset to another.
We demonstrate that there are two reasons for this trend.
Firstly, they over-fit on popular datasets in a traditional single-dataset training and test pipeline.
Secondly, the training source is generally not dense in pedestrians and diverse in scenarios.
Accordingly, through experiments we find that a general purpose object detector works better in direct cross-dataset evaluation compared with state-of-the-art pedestrian detectors and we illustrate that diverse and dense datasets, collected by crawling the web, serve to be an efficient source of pre-training for pedestrian detection.
Furthermore, we find that a progressive training pipeline works good for autonomous driving oriented detector.
We improve upon previous state-of-the-art on \textit{reasonable}/\textit{heavy} subsets of \emph{CityPersons} dataset by 1.3$\%$/1.7$\%$ and on \emph{Caltech} by 1.8$\%$/14.9$\%$ in terms of log average miss rate (\LMR{}) points without any fine-tuning on the test set. Detector trained through proposed pipeline achieves top rank at the leaderborads of \cityperson{} and \ecp{}. Code and models can be accessed at \url{https://github.com/hasanirtiza/Pedestron}.




\end{abstract}

==> sections/discussion.tex <==
\section{Discussion and Analysis} \label{sec:disc}
\subsection{Effect of Fine-tuning on Target Data}

With study presented in section \ref{sec:general-cap}, we find that existing methods may overfit on a single dataset, and so we suggest to put more emphasis on cross-dataset evaluation for a new way of benchmarking. However, to align to the previously established evaluation protocol on single dataset and compare to the existing state of the art, we conduct an additional study on fine-tuning our above models on target data. Experimental results show that, with progressively trained and generalizable baseline models, it is relatively more easy to adapt to new datasets by fine-tuning, and further performance gain can be achieved.

%  Therefore, we investigated the effect of pre-training on a large scale autonomous driving dataset along with fine-tuning on target dataset as reported in Table \ref{tab:finetune}. \emph{A} $\rightarrow$ \emph{B} refers to pre-training on \emph{A} and fine-tuning on the target dataset \emph{B}. Visible improvements can be seen in the case of \caltech{}, which resonates with our previous findings that due to low-resolution and sparse annotation, pre-training on \ecpa{} or \cityperson{} boosts the performances on \caltech{}. 
%  Importantly, in the case of \cityperson{}, the pre-training on \ecpa{} brings improvement of nearly 2$\%$ of \LMR{}, as discussed above, \ecpa{} brings density, both in terms of number of pedestrians and pedestrians per frame. Conversely, due to relative smaller size, the pre-training on \cityperson{} does not bring any improvements on \ecpa{}.
 
 

% On much challenging autonomous driving datasets such as \cityperson{} and \ecp{} as shown in Table \ref{tab:icon-ch-wider}, mere pre-training on diverse and dense pedestrian datasets does not result in any improvements compared to second and fifth row of Table \ref{tab:cross-cp-ecp-cal}. Since \crowdhuman{} and \widerperson{} though larger in diversity and density still are relatively under-represented in terms of only autonomous driving scenes, therefore fine-tuning on the target dataset is a necessity. 
% In Table \ref{tab:icon-finetune}, we present results of pre-training on a dataset and fine-tuning on the target dataset. \emph{A} $\rightarrow$ \emph{B} refers to pre-training on \emph{A} and fine-tuning on the target dataset \emph{B}. 
% Table \ref{tab:icon-finetune} shows that pre-training on a web-crawled dataset, with large diversity and density and subsequently fine-tuned on the target dataset provides significant improvements over only pre-training on the autonomous driving datasets and fine-tuning on the target datasets. 
% Improvements are consistent across all datasets and on all occlusion and size settings. 
% In comparison with Table \ref{tab:finetune}, where pre-training is done on autonomous driving datasets, improvement across all dataset (taking the best cases) are $3.3\%$, $0.4\%$ and $2.4\%$ of \LMR{} percentage points on \caltecha{}{}, \cityperson{} and \ecp{}, respectively. 
% Interestingly, \widerperson{} appears to be slightly better source of pre-training than \crowdhuman{} since it contains more images of autonomous driving scenes. 
% Finally, in Table \ref{tab:icon-finetune2}, starting with a pre-training on the web-crawled dataset, we fine-tuned our model on the largest autonomous driving dataset \ecp{} and subsequently fine-tuning on the target dataset. We refer to this as our \emph{progressive training pipeline}, results show that the best performances are achieved by using this training pipeline. Significant improvements across all datasets and under all evaluation settings can be observed using the progressive training pipeline where we eventually fine-tune on the target domain. Particularly, in comparison with \ref{tab:icon-finetune}, progressive pipeline improves upon previous performances on \textit{reasonable}/\textit{heavy} subsets of \emph{CityPersons} dataset by 1.6$\%$/14.4$\%$ and on \emph{Caltech} by 0.7$\%$/5.0$\%$ in terms of log average miss rate (\LMR{}) points.

% Note that though fine-tuning to a very specific domain does improve the performance on that domain, it requires human effort to annotate more data from that domain, and the obtained model may only be useful on that domain but on longer be generally effective on other domains. Therefore, to avoid human annotation in deployment of the detector and to keep a general model that can be applied to most scenarios, we still prefer to train a universal model and validate it by cross-dataset evaluation without adaptation on target data.






















% \begin{table}[t]
% %\parbox{.5\linewidth}{
% \centering
% \caption{Investigating  the performance of embedded vision model, when pre-trained on diverse and dense datasets.}
% \label{tab:mobileNet}
%   \resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
% \hline
% Training             & Reasonable & Small & Heavy \\ \hline
% CP    & 12.0     & 15.3     & 47.8 \\ \hline
% CrowdHuman$\rightarrow$CP  & 11.8   & 14.6   & 41.6   \\ \hline
% CrowdHuman$\rightarrow$ECP$\rightarrow$CP    &    10.9 & 14.4     &  44.6\\ \hline
% Wider Pedestrian$\rightarrow$CP  & 11.7     & 14.9   & 45.6   \\ \hline
% Wider Pedestrian$\rightarrow$ECP$\rightarrow$CP    & \textbf{10.1}    & \textbf{11.9}    & \textbf{35.4} \\ \hline
% \end{tabular}
% }
% %}
% \end{table}

% \begin{table}[t]

% %\parbox{.5\linewidth}{
% \centering
% \caption{WiderPerson split.}
% \label{tab:mobileNet}
% %\resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
% \hline
% Training             & Reasonable & Small & Heavy \\ \hline

% Wider-AD$\rightarrow$CP  &   &    &    \\ \hline
% Wider-AD$\rightarrow$ECP$\rightarrow$CP    &     &      & \\ \hline
% Wider-SUR$\rightarrow$CP  &      &    &   \\ \hline
% Wider-SUR$\rightarrow$ECP$\rightarrow$CP    &    &      & \\ \hline
% \end{tabular}
% %}
% %}
% \end{table}



% \subsection{Application Oriented Models}

% In many pedestrian detection applications, the size and computational cost of models is constrained.
% We experiment with a small and light-weight model MobileNet \cite{howard2017mobilenets}, which is designed for mobile and embedded vision applications, to investigate if the performance improvements hold true.
% %We investigated a light-weight mobile and embedded vision application oriented model MobileNet \cite{howard2017mobilenets}, providing fast speed and fewer hyper-parameters, thus tailor-made for practical applications. 
% Table \ref{tab:mobileNet} shows results on \cityperson{} using \mobnet{} as a backbone network architecture into our baseline. 
% Intuitively, \mobnet{} performs worse than the HRNet \cite{wang2019deep}. 
% However, in the case of \mobnet{} as well, we see pre-training on \crowdhuman{} and fine-tuning on \cityperson{} improves the performance of the \mobnet{}. 
% Subsequently, we pre-train (3rd row) \mobnet{} on \crowdhuman{} and \ecp{} before fine-tuning on \cityperson{}. 
% Improvement of nearly 1$\%$ of \LMR{} can be observed. 
% Furthermore, we replaced \crowdhuman{} with \widerperson{} as the initial source of pre-training. Improvement over the baseline (1st row) can be observed (4th row). 
% Importantly, in the last row of Table \ref{tab:mobileNet}, largest gain can be observed. 
% This is consistent with our previous finding reported in Table \ref{tab:icon-finetune2}, \widerperson{} is a better source of pre-training than \crowdhuman{}, since it has images of autonomous driving scenes as well making it more diverse than \crowdhuman{}. 
% Interestingly, in the case of \crowdhuman{} and \widerperson{}, even with a light-weight architecture, our baseline outperformed state-of-the-art pedestrian detector CSP \cite{Liu2018DBC}. 
% In summary, even with a light weight back-bone architecture, by pre-training on diverse and dense datasets, \mobnet{} outperformed previous best performing method on \cityperson{}, i.e. CSP \cite{Liu2018DBC}.  


% \subsection{Failure Cases}

% \begin{figure}[tbh]
% \begin{subfigure}{0.19\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-easy/amsterdam_01217.jpg}
%   \caption{}
%   \label{fig:failures:fp:easy1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.16\textwidth}
%   \centering
%   \includegraphics[height=0.19\textheight]{images/fp-easy/barcelona_01488.jpg}  
%   \caption{}
%   \label{fig:failures:fp:easy2}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/barcelona_01504.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno1}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/bologna_01299.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno2}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/bologna_01364.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno3}
% \end{subfigure}

% \vspace{-0.25cm}
% \begin{subfigure}{0.11\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/amsterdam_01140.jpg}  
%   \caption{}
%   \label{fig:failures:fn:1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.21\textwidth}
%   \centering
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01444.jpg}  
%   \caption{}
%   \label{fig:failures:fn:2}
% \end{subfigure}
% \begin{subfigure}{0.21\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01283.jpg}  
%   \caption{}
%   \label{fig:failures:fn:3}
% \end{subfigure}
% \begin{subfigure}{0.19\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01336.jpg}  
%   \caption{}
%   \label{fig:failures:fn:4}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/basel_00692.jpg}  
%   \caption{}
%   \label{fig:failures:fn:5}
% \end{subfigure}
% \vspace{-0.6cm}
% \caption{Failure cases for Cascade R-CNN\textsuperscript{$\dagger$} on EuroCityPersons at 0.1 false positive per image.
% Top row: False positives. Bottom row: False negatives.}
% \label{fig:failures}
% \end{figure}


% % \todo{selected errors: \url{https://drive.google.com/open?id=1ELtQ-4_8CDPRtSG-08wDJVpifb4dGnZU}}
% Most of the errors of our best model are quite challenging cases either due to large occlusion, small size of the pedestrian, low illumination and/or the presence of another pedestrian in the vicinity, which leads to the bounding box of the pedestrian being deleted as has been reported previously \cite{braun2018eurocity}.
% In Fig.\ref{fig:failures}, we shows some examples of the easiest (for a human) false negatives (FN) and false positives (FP) samples at 0.1 FP per image.
% Some FPs, Fig.\ref{fig:failures:fp:easy1}-\ref{fig:failures:fp:easy2}, are due to depictions of people in pictures, and due to shadows and objects which slightly resemble a pedestrian but the model fails to correctly classify them.
% We also show few false positives in Fig.\ref{fig:failures:fp:anno1}-\ref{fig:failures:fp:anno3}, which are due to annotation mistakes.
% Even though, most false negatives are difficult even for a human, the model nevertheless sometimes fails to detect relatively easy (large, non-occluded) pedestrians and the cause of many of these failure is not obvious.
% Fig.\ref{fig:failures:fn:1}-\ref{fig:failures:fn:5} shows some of these cases.

% Most of the failures of the model are extremely challenging cases, where it is difficult to determine whether the false positives (FPs) are actually a pedestrian and the annotators have missed them or the model has made a mistake and cases where the shadow or background objects look similar to a pedestrian.
% Similarly, most of the False negatives (FNs) are pedestrians which are heavily occluded, with only a small part of pedestrian is visible.

% Even though most of the errors are very challenging cases, there are nevertheless some easy but uncommon cases where the model fails to detect pedestrians, e.g person sitting in a car, on a bench, or in a construction vehicle, etc. or detects pedestrians in background, e.g. picture on the side of a vehicle, etc.

% There are also some cases where the pedestrian is un-occluded and quite large, but the model still fails, so even though the proposed model improves performance considerably, it nevertheless can fail for some relatively easy cases.



==> sections/discussion_old.tex <==
\section{Discussion and Analysis} \label{sec:disc}
\subsection{Effect of Fine-tuning on Target Data}

With study presented in section \ref{sec:general-cap}, we find that existing methods may overfit on a single dataset, and so we suggest to put more emphasis on cross-dataset evaluation for a new way of benchmarking. However, to align to the previously established evaluation protocol on single dataset and compare to the existing state of the art, we conduct an additional study on fine-tuning our above models on target data. Experimental results show that, with progressively trained and generalizable baseline models, it is relatively more easy to adapt to new datasets by fine-tuning, and further performance gain can be achieved.

 Therefore, we investigated the effect of pre-training on a large scale autonomous driving dataset along with fine-tuning on target dataset as reported in Table \ref{tab:finetune}. \emph{A} $\rightarrow$ \emph{B} refers to pre-training on \emph{A} and fine-tuning on the target dataset \emph{B}. Visible improvements can be seen in the case of \caltech{}, which resonates with our previous findings that due to low-resolution and sparse annotation, pre-training on \ecpa{} or \cityperson{} boosts the performances on \caltech{}. 
 Importantly, in the case of \cityperson{}, the pre-training on \ecpa{} brings improvement of nearly 2$\%$ of \LMR{}, as discussed above, \ecpa{} brings density, both in terms of number of pedestrians and pedestrians per frame. Conversely, due to relative smaller size, the pre-training on \cityperson{} does not bring any improvements on \ecpa{}.
 
 
 \begin{table}[tb]
\centering
\caption{Showing how well CityPersons (CP) and ECP are as the source of pre-training.}
\label{tab:finetune}
\begin{tabular}{l|c|c|c}
\hline
Training             & Reasonable & Small & Heavy \\ \hline
CP$\rightarrow$Caltech    & 5.9   & 8.6      & 27.0 \\ \hline
ECP$\rightarrow$Caltech    &  5.7 & 7.7      & 26.8  \\ \hline
CP$\rightarrow$ECP    &  6.8   & 12.3     & 33.0\\ \hline
ECP$\rightarrow$CP  & 9.59   &    11.04 & 36.0  \\ \hline
\end{tabular}
\end{table}
 
On much challenging autonomous driving datasets such as \cityperson{} and \ecp{} as shown in Table \ref{tab:icon-ch-wider}, mere pre-training on diverse and dense pedestrian datasets does not result in any improvements compared to second and fifth row of Table \ref{tab:cross-cp-ecp-cal}. Since \crowdhuman{} and \widerperson{} though larger in diversity and density still are relatively under-represented in terms of only autonomous driving scenes, therefore fine-tuning on the target dataset is a necessity. 
In Table \ref{tab:icon-finetune}, we present results of pre-training on a dataset and fine-tuning on the target dataset. \emph{A} $\rightarrow$ \emph{B} refers to pre-training on \emph{A} and fine-tuning on the target dataset \emph{B}. 
Table \ref{tab:icon-finetune} shows that pre-training on a web-crawled dataset, with large diversity and density and subsequently fine-tuned on the target dataset provides significant improvements over only pre-training on the autonomous driving datasets and fine-tuning on the target datasets. 
Improvements are consistent across all datasets and on all occlusion and size settings. 
In comparison with Table \ref{tab:finetune}, where pre-training is done on autonomous driving datasets, improvement across all dataset (taking the best cases) are $3.3\%$, $0.4\%$ and $2.4\%$ of \LMR{} percentage points on \caltecha{}{}, \cityperson{} and \ecp{}, respectively. 
Interestingly, \widerperson{} appears to be slightly better source of pre-training than \crowdhuman{} since it contains more images of autonomous driving scenes. 
Finally, in Table \ref{tab:icon-finetune2}, starting with a pre-training on the web-crawled dataset, we fine-tuned our model on the largest autonomous driving dataset \ecp{} and subsequently fine-tuning on the target dataset. We refer to this as our \emph{progressive training pipeline}, results show that the best performances are achieved by using this training pipeline. Significant improvements across all datasets and under all evaluation settings can be observed using the progressive training pipeline where we eventually fine-tune on the target domain. Particularly, in comparison with \ref{tab:icon-finetune}, progressive pipeline improves upon previous performances on \textit{reasonable}/\textit{heavy} subsets of \emph{CityPersons} dataset by 1.6$\%$/14.4$\%$ and on \emph{Caltech} by 0.7$\%$/5.0$\%$ in terms of log average miss rate (\LMR{}) points.

Note that though fine-tuning to a very specific domain does improve the performance on that domain, it requires human effort to annotate more data from that domain, and the obtained model may only be useful on that domain but on longer be generally effective on other domains. Therefore, to avoid human annotation in deployment of the detector and to keep a general model that can be applied to most scenarios, we still prefer to train a universal model and validate it by cross-dataset evaluation without adaptation on target data.


\begin{table}[tb]
\centering
\caption{Illustrating how our baseline behave with fine-tuning on the target dataset when CrowdHuman and Wider Pedestrian are used as a source of pre-training.}
\label{tab:icon-finetune}
 \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Training             & Reasonable & Small & Heavy \\ \hline
CrowdHuman$\rightarrow$Caltech    &  2.7    &  10.9     & 31.0  \\ \hline
Wider Pedestrian$\rightarrow$Caltech    & \textbf{2.4}  &   \textbf{9.8}   & \textbf{30.7}  \\ \hline
\hline
CrowdHuman$\rightarrow$CP    &  9.2   & 14.7      & 38.02\\ \hline
Wider Pedestrian$\rightarrow$CP  &  \textbf{9.1}  & \textbf{11.0}     & \textbf{34.4}   \\ \hline
\hline
CrowdHuman$\rightarrow$ECP    &  4.5   &   9.3   & 23.0 \\ \hline
Wider Pedestrian$\rightarrow$ECP  &  \textbf{4.4}    &  \textbf{9.1}   & \textbf{21.3}  \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[tb]
\centering
\caption{Showing the effect of fine-tuning in a cascaded manner.}
\label{tab:icon-finetune2}
 \resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Training             & Reasonable & Small & Heavy \\ \hline
ECP$\rightarrow$Caltech    &    5.7 & 7.7     & 26.8  \\ \hline
CrowdHuman$\rightarrow$ECP$\rightarrow$Caltech    & 2.2     &   8.1   & 30.7 \\ \hline
Wider Pedestrian$\rightarrow$ECP$\rightarrow$Caltech    &  \textbf{1.7}  & \textbf{7.2}     & \textbf{25.7}\\ \hline
\hline
ECP$\rightarrow$CP  & 9.5     & 11.0   & 36.0  \\ \hline
CrowdHuman$\rightarrow$ECP$\rightarrow$CP  & 8.0     & 8.5   & 27.0  \\ \hline
Wider Pedestrian$\rightarrow$ECP$\rightarrow$CP  & \textbf{7.5}     & \textbf{8.0}    & \textbf{28.0}  \\ \hline
\end{tabular}
}
\end{table}



\subsection{Comparison with Current State-of-the-Art}
In this section we present a comparative analysis of state-of-the-art of pedestrian detection. For our comparative analysis, we choose the best performing pedestrian detectors on \caltech{} and \cityperson{}. The underlying goal is to illustrate how well our baseline performs when it is fine-tune on the target dataset.
We refer to the best performing baseline presented in Table \ref{tab:icon-finetune2} as \textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$}. 
Table \ref{tab:Caltech-SOTA} shows that \textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$} achieves 1.76 \LMR{} on \caltech{}, outperforming previous best by a margin of $3.24\%$ of \LMR{}. 
This performance is approaching \emph{human-baseline} (0.88) \cite{zhang2016far} on \caltech{} .
Moreover, we report similar improvement over the previous state-of-the-art on \cityperson{} benchmark. \textbf{\emph{Cascade R-CNN's}}\textsuperscript{$\dagger$} performance is $3.5\%$ \LMR{} better than CSP \cite{Liu2018DBC}. 
Finally, on \ecp{} we report an improvements of $1.8\%$ \LMR{} over Faster R-CNN \cite{ren2015faster}. 
Similar performance improvements are achieved on other subsets of all these three datasets, with the performance improvement of more than 50\% for the most challenging subsets, \textit{Heavy} and \textit{small}.
This consistent improvement over all datasets illustrates the robustness of the \textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$}, as it significantly outperform previous state-of-the-art.

\begin{table}[tb]
\centering
\caption{Comparison with state-of-the-art on Caltech.}
\label{tab:Caltech-SOTA}
%  \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Method         & Reasonable & Heavy & All  \\ \hline
DeepParts\cite{tian2015deep}       & 11.89      & 60.42 & --   \\ \hline
CompactACT-Deep\cite{cai2015learning} & 9.2        & --    & --   \\ \hline
FRCNN\cite{zhang2017citypersons}           & 8.7        & 53.1  & 62.6 \\ \hline
RPN +BF\cite{zhang2016faster}         & 7.3        & 54.6  & 59.9 \\ \hline
ALFNet\cite{liu2018learning}          & 6.1        & 51.0  & 59.1 \\ \hline
Hyper Learner\cite{mao2017can}   & 5.5        & 48.7  & 61.5 \\ \hline
Rep Loss\cite{wang2018repulsion}        & 5.0        & 47.9  & 59.0 \\ \hline
CSP\cite{Liu2018DBC}   & 5.8        & 46.6  & 57.7 \\ \hline
\textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$}        & \textbf{1.7}        & \textbf{25.7}  &\textbf{ 27.4} \\ \hline
\end{tabular}
%}
\end{table}

\begin{table}[]
\centering
\caption{Comparison with state-of-the-art on ECP. The results are evaluated on the testing set.}
\label{tab:ECP-SOTA}
%  \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Method             & Reasonable & Small & Heavy \\ \hline
Faster R-CNN    & 7.3  & 16.6     & 52.0 \\ \hline
YOLOv3    &  8.5 & 17.8     & 37.0\\ \hline
SSD &  10.5 & 20.5   & 42.0 \\ \hline
\textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$} & \textbf{5.5}    & \textbf{11.7}   & \textbf{26.1} \\ \hline
\end{tabular}
%}
\end{table}



\begin{table*}[ht]
\begin{center}
\caption{Comparison with state-of-the-art on CityPersons.}
\label{tab:City-SOTA}
\resizebox{.999\textwidth}{!}{
\begin{tabular}{c|c|c|c c c|c c c|c}
\hline
Method & Backbone & Reasonable & Heavy*  & Partial & Bare & Small & Medium & Large & Test Time\\
\hline
\hline
FRCNN\cite{zhang2017citypersons} & VGG-16 & 15.4 & - & - & - & 25.6 & 7.2 & 7.9 & -\\
\hline
RetinaNet \cite{lin2017focal}  & ResNet-50 & 15.6 & 49.9 & - & - & - & - & - & -\\
\hline
CornerNet \cite{Law_2018_ECCV} & Hourglass-54 & 21.0 & 56.0 & - & - & - & - & - & -\\
\hline
FRCNN+Seg\cite{zhang2017citypersons} & VGG-16 & 14.8 & - & - & - & 22.6 & 6.7 & 8.0 & -\\
\hline
OR-CNN\cite{zhang2018occlusion} & VGG-16 & 12.8 & 55.7 & 15.3 & 6.7 & - & - & - & -\\
\hline
RepLoss\cite{wang2018repulsion} & ResNet-50 & 13.2 & 56.9 & 16.8 & 7.6 & - & - & -& -\\
\hline
TLL\cite{song2018small} & ResNet-50 & 15.5 & 53.6 & 17.2 & 10.0 & - & - & -& -\\
\hline
TLL+MRF\cite{song2018small} & ResNet-50 & 14.4 & 52.0 & 15.9 & 9.2 & - & - & -& -\\
\hline
ALFNet\cite{liu2018learning} & ResNet-50 & 12.0 & 51.9 & 11.4 & 8.4 & 19.0 & 5.7 & 6.6 & 0.27s/img\\
\hline
CSP\cite{Liu2018DBC} & ResNet-50 & {11.0} & 49.3 & 10.4 & {7.3} & {16.0} & {3.7} & {6.5}& 0.33s/img\\
\hline
\textbf{\emph{Cascade R-CNN}}\textsuperscript{$\dagger$} & HRNet & \textbf{{7.5}} & \textbf{{33.9}} & \textbf{5.7} & \textbf{6.2} & \textbf{8.0} & \textbf{3.0} & \textbf{4.3}  & 0.33s/img\\
\hline
\end{tabular}
}
\end{center}

\end{table*}










\begin{table}[t]
%\parbox{.5\linewidth}{
\centering
\caption{Investigating  the performance of embedded vision model, when pre-trained on diverse and dense datasets.}
\label{tab:mobileNet}
  \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
Training             & Reasonable & Small & Heavy \\ \hline
CP    & 12.0     & 15.3     & 47.8 \\ \hline
CrowdHuman$\rightarrow$CP  & 11.8   & 14.6   & 41.6   \\ \hline
CrowdHuman$\rightarrow$ECP$\rightarrow$CP    &    10.9 & 14.4     &  44.6\\ \hline
Wider Pedestrian$\rightarrow$CP  & 11.7     & 14.9   & 45.6   \\ \hline
Wider Pedestrian$\rightarrow$ECP$\rightarrow$CP    & \textbf{10.1}    & \textbf{11.9}    & \textbf{35.4} \\ \hline
\end{tabular}
}
%}
\end{table}

% \begin{table}[t]

% %\parbox{.5\linewidth}{
% \centering
% \caption{WiderPerson split.}
% \label{tab:mobileNet}
% %\resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
% \hline
% Training             & Reasonable & Small & Heavy \\ \hline

% Wider-AD$\rightarrow$CP  &   &    &    \\ \hline
% Wider-AD$\rightarrow$ECP$\rightarrow$CP    &     &      & \\ \hline
% Wider-SUR$\rightarrow$CP  &      &    &   \\ \hline
% Wider-SUR$\rightarrow$ECP$\rightarrow$CP    &    &      & \\ \hline
% \end{tabular}
% %}
% %}
% \end{table}



% \subsection{Application Oriented Models}

% In many pedestrian detection applications, the size and computational cost of models is constrained.
% We experiment with a small and light-weight model MobileNet \cite{howard2017mobilenets}, which is designed for mobile and embedded vision applications, to investigate if the performance improvements hold true.
% %We investigated a light-weight mobile and embedded vision application oriented model MobileNet \cite{howard2017mobilenets}, providing fast speed and fewer hyper-parameters, thus tailor-made for practical applications. 
% Table \ref{tab:mobileNet} shows results on \cityperson{} using \mobnet{} as a backbone network architecture into our baseline. 
% Intuitively, \mobnet{} performs worse than the HRNet \cite{wang2019deep}. 
% However, in the case of \mobnet{} as well, we see pre-training on \crowdhuman{} and fine-tuning on \cityperson{} improves the performance of the \mobnet{}. 
% Subsequently, we pre-train (3rd row) \mobnet{} on \crowdhuman{} and \ecp{} before fine-tuning on \cityperson{}. 
% Improvement of nearly 1$\%$ of \LMR{} can be observed. 
% Furthermore, we replaced \crowdhuman{} with \widerperson{} as the initial source of pre-training. Improvement over the baseline (1st row) can be observed (4th row). 
% Importantly, in the last row of Table \ref{tab:mobileNet}, largest gain can be observed. 
% This is consistent with our previous finding reported in Table \ref{tab:icon-finetune2}, \widerperson{} is a better source of pre-training than \crowdhuman{}, since it has images of autonomous driving scenes as well making it more diverse than \crowdhuman{}. 
% Interestingly, in the case of \crowdhuman{} and \widerperson{}, even with a light-weight architecture, our baseline outperformed state-of-the-art pedestrian detector CSP \cite{Liu2018DBC}. 
% In summary, even with a light weight back-bone architecture, by pre-training on diverse and dense datasets, \mobnet{} outperformed previous best performing method on \cityperson{}, i.e. CSP \cite{Liu2018DBC}.  


% \subsection{Failure Cases}

% \begin{figure}[tbh]
% \begin{subfigure}{0.19\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-easy/amsterdam_01217.jpg}
%   \caption{}
%   \label{fig:failures:fp:easy1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.16\textwidth}
%   \centering
%   \includegraphics[height=0.19\textheight]{images/fp-easy/barcelona_01488.jpg}  
%   \caption{}
%   \label{fig:failures:fp:easy2}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/barcelona_01504.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno1}
% \end{subfigure}
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/bologna_01299.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno2}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fp-anno/bologna_01364.jpg}
%   \caption{}
%   \label{fig:failures:fp:anno3}
% \end{subfigure}

% \vspace{-0.25cm}
% \begin{subfigure}{0.11\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/amsterdam_01140.jpg}  
%   \caption{}
%   \label{fig:failures:fn:1}
% \end{subfigure}
% \bigskip % force a bit of vertical whitespace
% \begin{subfigure}{0.21\textwidth}
%   \centering
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01444.jpg}  
%   \caption{}
%   \label{fig:failures:fn:2}
% \end{subfigure}
% \begin{subfigure}{0.21\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01283.jpg}  
%   \caption{}
%   \label{fig:failures:fn:3}
% \end{subfigure}
% \begin{subfigure}{0.19\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/barcelona_01336.jpg}  
%   \caption{}
%   \label{fig:failures:fn:4}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   % include first image
%   \includegraphics[height=0.19\textheight]{images/fn-easy/basel_00692.jpg}  
%   \caption{}
%   \label{fig:failures:fn:5}
% \end{subfigure}
% \vspace{-0.6cm}
% \caption{Failure cases for Cascade R-CNN\textsuperscript{$\dagger$} on EuroCityPersons at 0.1 false positive per image.
% Top row: False positives. Bottom row: False negatives.}
% \label{fig:failures}
% \end{figure}


% % \todo{selected errors: \url{https://drive.google.com/open?id=1ELtQ-4_8CDPRtSG-08wDJVpifb4dGnZU}}
% Most of the errors of our best model are quite challenging cases either due to large occlusion, small size of the pedestrian, low illumination and/or the presence of another pedestrian in the vicinity, which leads to the bounding box of the pedestrian being deleted as has been reported previously \cite{braun2018eurocity}.
% In Fig.\ref{fig:failures}, we shows some examples of the easiest (for a human) false negatives (FN) and false positives (FP) samples at 0.1 FP per image.
% Some FPs, Fig.\ref{fig:failures:fp:easy1}-\ref{fig:failures:fp:easy2}, are due to depictions of people in pictures, and due to shadows and objects which slightly resemble a pedestrian but the model fails to correctly classify them.
% We also show few false positives in Fig.\ref{fig:failures:fp:anno1}-\ref{fig:failures:fp:anno3}, which are due to annotation mistakes.
% Even though, most false negatives are difficult even for a human, the model nevertheless sometimes fails to detect relatively easy (large, non-occluded) pedestrians and the cause of many of these failure is not obvious.
% Fig.\ref{fig:failures:fn:1}-\ref{fig:failures:fn:5} shows some of these cases.

% Most of the failures of the model are extremely challenging cases, where it is difficult to determine whether the false positives (FPs) are actually a pedestrian and the annotators have missed them or the model has made a mistake and cases where the shadow or background objects look similar to a pedestrian.
% Similarly, most of the False negatives (FNs) are pedestrians which are heavily occluded, with only a small part of pedestrian is visible.

% Even though most of the errors are very challenging cases, there are nevertheless some easy but uncommon cases where the model fails to detect pedestrians, e.g person sitting in a car, on a bench, or in a construction vehicle, etc. or detects pedestrians in background, e.g. picture on the side of a vehicle, etc.

% There are also some cases where the pedestrian is un-occluded and quite large, but the model still fails, so even though the proposed model improves performance considerably, it nevertheless can fail for some relatively easy cases.


